Can Copyright be Reduced to Privacy?

There is a growing concern that generative AI models will generate outputs closely resembling the copyrighted materials for which they are trained. This worry has intensified as the quality and complexity of generative models have immensely improved, and the availability of extensive datasets containing copyrighted material has expanded. Researchers are actively exploring strategies to mitigate the risk of generating infringing samples, with a recent line of work suggesting to employ techniques such as differential privacy and other forms of algorithmic stability to provide guarantees on the lack of infringing copying. In this work, we examine whether such algorithmic stability techniques are suitable to ensure the responsible use of generative models without inadvertently violating copyright laws. We argue that while these techniques aim to verify the presence of identifiable information in datasets, thus being privacy-oriented, copyright law aims to promote the use of original works for the benefit of society as a whole, provided that no unlicensed use of protected expression occurred. These fundamental differences between privacy and copyright must not be overlooked. In particular, we demonstrate that while algorithmic stability may be perceived as a practical tool to detect copying, such copying does not necessarily constitute copyright infringement. Therefore, if adopted as a standard for detecting an establishing copyright infringement, algorithmic stability may undermine the intended objectives of copyright law.

==> header_iclr.tex <==
\usepackage{amsmath,amsfonts,amsthm,amssymb}
\usepackage{mathtools,cancel}
\usepackage{thmtools, amssymb}
\usepackage{bbm}
\usepackage{algorithm}
\usepackage{xcolor}
\usepackage[noend]{algpseudocode}
\usepackage{mdframed}
\usepackage{caption}
\usepackage{xspace}

% New Century Schoolbook
% \usepackage{scholax}
% % \usepackage{tgschola}
% \usepackage[scaled=1.0,ncf,vvarbb]{newtxmath}
% \usepackage{thmtools,thm-restate}
%\usepackage[colorlinks,allcolors=blue]{hyperref}
%\usepackage{enumitem}
\newcommand{\labelthis}[1]{\stepcounter{equation}\tag{\theequation}\label{#1}}
\usepackage[capitalise]{cleveref}
\newcommand{\hist}{\mathrm{hist}}
\declaretheorem{theorem}
\newtheorem{problem}{Open Question}
\newtheorem*{theorem*}{Theorem}
\newtheorem{proposition}{Proposition}
\newtheorem*{corollary*}{Corollary}
\declaretheorem[sibling=theorem]{lemma}
\declaretheorem[sibling=theorem]{corollary}
\declaretheorem[sibling=theorem]{claim}
\declaretheorem[sibling=theorem]{observation}
\declaretheorem[sibling=theorem,style=definition]{definition}
\declaretheorem[sibling=theorem,style=remark]{remark}
\let\proof\undefined
\declaretheoremstyle[
        spaceabove=\topsep, 
        spacebelow=\topsep, 
        % headfont=\normalfont\bfseries,
        bodyfont=\normalfont,
        notefont=\normalfont\bfseries,
        % notebraces={(}{)},
        notebraces={}{},
        % postheadspace=0.33em, 
        qed=$\blacksquare$, 
        % headpunct={},
        % postfoothook=\noindent\ignorespaces
    ]{proofstyle}
\declaretheorem[style=proofstyle,numbered=no,name=Proof]{proof}

\usepackage{xcolor}
\usepackage[extdef=true]{delimset}

\usepackage{crossreftools}

\pdfstringdefDisableCommands{%
    \let\Cref\crtCref
    \let\cref\crtcref
}

\crefname{claim}{Claim}{Claims}
\newcommand{\safe}{\mathrm{safe}}
\newcommand{\naf}{\mathrm{NAF}}
\newcommand{\cD}{\mathcal{D}}

% \usepackage[todonotes={textsize=footnotesize}]{changes}
% % \usepackage[final]{changes}
% \definechangesauthor[name=TK]{TK}
% \definechangesauthor[name=RL,color=magenta]{RL}
% \definechangesauthor[name=IA,color=teal]{IA}



% some defs

\newcommand{\reals}{\mathbb{R}}
\DeclareMathOperator*{\spn}{span}
\DeclareMathOperator*{\spnb}{span^{\mathcal{B}_r}}
\DeclareMathOperator*{\spnone}{span^{1}}
\newcommand{\W}{\mathcal{W}}
\renewcommand{\E}{\mathop{\mathbb{E}}}
\newcommand{\dotp}{\boldsymbol{\cdot}}
\newcommand{\hsep}{\vspace{2ex}\noindent\rule{\textwidth}{1pt}\vspace{2ex}}

\DeclareMathOperator*{\rem}{remainder}

\DeclarePairedDelimiter\bigceil{\big\lceil}{\big\rceil}
\DeclarePairedDelimiter\Bigceil{\Big\lceil}{\Big\rceil}

\DeclarePairedDelimiter\bigfloor{\Big\lfloor}{\Big\rfloor}
\newcommand{\wrgd}{w^{\lambda\textrm{GD}}}
\newcommand{\wgd}{w^{\textrm{GD}}}
\newcommand{\wsgd}{w^{\textrm{SGD}}}
\newcommand{\etabar}{\overline\eta}
\newcommand{\wbar}{\overline{w}}
\newcommand{\vbar}{\bar{v}}
\newcommand{\X}{\mathcal{X}}
\newcommand{\add}[1]{\textbf{#1}}
\newcommand{\betabar}{\bar{\beta}}
\newcommand{\wt}[1]{\widetilde{#1}}
\newcommand{\wh}[1]{\widehat{#1}}
\newcommand{\s}{\mathbf{s}}
\renewcommand{\R}{\mathbb{R}}
\renewcommand{\P}{\mathbb{P}}
\newcommand{\regret}{\mathcal{R}_T}
\newcommand{\OurAlgorithm}{Switch Tsallis, Switch!}
\newcommand{\pregret}{\overline{\mathcal{R}}_T}
\newcommand{\regretsw}{\mathcal{R}^\lambda_T}
\newcommand{\pregretsw}{\overline{\mathcal{R}}^\lambda_T}
\newcommand{\regretn}[1]{\mathcal{R}^{(#1)}}
\newcommand{\pregretn}[1]{\overline{\mathcal{R}}^{(#1)}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\Deltamin}{\Delta_{\textrm{min}}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\Q}{\mathcal{Q}}
\newcommand{\cI}{\mathcal{I}(S)}
\newcommand{\cIt}[1]{\mathcal{I}_{#1}(S)}
\newcommand{\cIminus}{\mathcal{I}^-}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\F}{\mathcal{F}}
\newcommand{\medcup}{\textstyle \bigcup}
\newcommand{\Z}{\mathcal{Z}}
\newcommand{\epsilonbold}{\boldsymbol{\epsilon}}
\newcommand{\indicator}{\mathbbm{1}}
\newcommand{\totalvar}{d_{\textrm{TV}}^\F}
\newcommand{\discolorlinks}[1]{{\hypersetup{hidelinks}#1}}
\newcommand{\D}{\mathcal{D}}
\newcommand{\red}[1]{{\color{red}{#1}}}
\newcommand{\ignore}[1]{}
\newcommand{\Sexc}[2]{#1^{\backslash #2}}
\newcommand{\Si}{\Sexc{S}{i}}
\newcommand{\grad}{\nabla}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\bP}{\mathbb{P}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\construct}[1]{\f{\discolorlinks{\ref{#1}}}}
\newcommand{\ffull}{\construct{eq:construction}}
\newcommand{\fsimple}{\construct{eq:construction_simple}}

\renewcommand{\rl}[1]{{\color{red}\bfseries{RL: #1}}}
\newcommand{\sm}[1]
{{\color{red}\bfseries{SM: #1}}}
\newcommand{\niv}[1]
{{\color{blue}\bfseries{NE: #1}}}
\newcommand{\uh}[1]
{{\color{blue}\bfseries{UH: #1}}}
% \newcommand{\ia}[1]{{\color{green!75!black}\bfseries{IA: #1}}}
% \newcommand{\tk}[1]{{\color{magenta}\bfseries{TK: #1}}}
% \newcommand{\ga}[1]{{\color{cyan!75!black}\bfseries{GA: #1}}}

==> merge.tex <==


\begin{abstract}
There is a growing concern that generative AI models may generate outputs that closely resemble the copyrighted input content used for their training.  This worry has intensified as the quality and complexity of generative models have immensely improved, and the availability of extensive datasets containing copyrighted material has expanded. Researchers are actively exploring strategies to mitigate the risk of producing infringing samples, and a recent line of work suggests employing techniques such as differential privacy and other forms of algorithmic stability to safeguard copyrighted content.
In this work, we examine whether algorithmic stability techniques such as differential privacy are suitable to ensure the responsible use of generative models without inadvertently violating copyright laws. We argue that there are fundamental differences between privacy and copyright that should not be overlooked. In particular, we highlight that although algorithmic stability may be perceived as a practical tool to detect copying, it does not necessarily equate to copyright protection. Therefore, if it is adopted as a standard for copyright infringement, it may undermine the intended purposes of copyright law
 
\end{abstract}


\section{Introduction}
Recent advancements in Machine Learning have sparked a wave of new possibilities and applications that could potentially transform various aspects of our daily lives and revolutionize numerous professions through automation. However, training such algorithms relies heavily on extensive content,


==================================
which may include copyrighted materials. Under U.S. copyright law, copyright protection subsists in original works of authorship fixed in any tangible medium of expression (17 U.S.C. § 102(a)), excluding any “idea, procedure, process, system, method of operation, concept, principle, or discovery, regardless of the form in which it is described, explained, illustrated, or embodied in such work." (17 U.S.C. § 102(b). The unauthorized copying of copyrighted works may amount to copyright infringement (17 U.S.C. § 106) unless permitted by exceptions and limitations provided by law (17 U.S.C. §107-122; Pamela Samuelson, Generative AI meets copyright, 381 Science 6654 (2023)] Consequently, identifying and 




=================================================
determining when and how content can be used within this framework without infringing upon individuals’ legal rights has become a pressing challenge. Foundation Models and generative AI (GenAI), which are trained on gigantic datasets, exacerbate this challenge.  One area where this issue arises prominently is in the operation of generative models, which take human-produced content—much of it copyrighted– as input and are expected to generate ”similar” content. For instance, consider a machine that is trained on images and then generates new images that resemble the images it was trained on. In this context, the fundamental question arises:
When does the content generated by a machine (output content) infringe copyright in the training set (input content)?
This question is not purely theoretical, as various aspects of this problem have become subjects of legal disputes in recent years. In 2022, a class action was filed against Microsoft, GitHub, and OpenAI, claiming that their code-generating systems, Codex and Copilot, infringed copyright in the licensed code on which the system was allegedly trained (Complaint Class Action & Demand for Jury Trial, Doe 1 v. GitHub, Inc., No. 06823 (N.D. Cal. Nov. 3, 2022)). Similarly, in another class action against Stable Diffusion, Midjourney, and DeviantArt, plaintiffs argue that by training their system on web-scraped images, the defendant infringes the rights of millions of artists. Allegedly, the images these systems produce, in response to prompts provided by the systems’ users, are based entirely on the training images, which belong to plaintiffs, and, as such, are considered unauthorized derivative works of the plaintiffs’ images [17 US Code § 106 (2)].
A preliminary question that arises is whether it is lawful to use copyrighted content in the course of training [24, 29, 30]. Compelling arguments suggest that such intermediary copying might be considered fair use. In two fair use decisions involving the mass digitization of copyrighted books from university library collections to create a searchable database of millions of books, the Court of Appeals for the Second Circuit held that such practice was considered fair use [2] (Authors Guild, Inc. v. HathiTrust Authors Guild, Inc. v. Google, Inc.). 
A different claim is that generative models reproduce protected copyright expressions from the input content on which the model was trained in responding to users’ prompts. To claim that the output content of generative models infringes her copyright, a plaintiff must prove that the model had access to the protected expression that originated from her work and that the alleged copy is substantially similar to her work (Sid & Marty Krofft TV Prod., Inc. v. McDonald's Corp., 562 F.2d 1157, 1164 (9th Cir. 1977)).
To address these challenges, recent studies have proposed measurable metrics to quantify the finding of a copyright infringement [15, 17, 36, 38]. One approach [15, 38] asserts that copyright infringement does not occur if it is plausible for a machine to generate the output content without access to the input content. This argument can be illustrated as follows: Suppose Alice generates content A and Bob claims it plagiarizes content B. Alice might assert that she never saw content B thus implying that she did not infringe Bob’s copyright. However, since Alice must have observed some content, a secondary line of defense could be that  “had she never seen B” she would still be likely to generate A. This argument was exemplified by Bousquet et al. [15], that interpret differential privacy in the above manner. Subsequently, Vyas et al. [38] presented a specific generalization, in the form of a near-free access (NAF) notion that can potentially allow a more versatile notion of copyright protection.
These notations tend to oversimplify copyright law, inaccurately equating it with privacy concerns.  To begin with, an essential element of copyright law in the United States is its utilitarian rationale, seeking to promote the creation and deployment of creative works [5, 9]. It is crucial, then, that any interpretation of copyright, or any quantifiable measure for copyright, will be aligned with these objectives. In particular, while the law delineates a set of exclusive rights to the creators of original expressions, it must ensure sufficient creative space for current and future creators [35]. 
Crucial issues distinguish copyright law from privacy as defined by criteria such as algorithmic stability. First, copyright is limited in time, and once protection has expired, the work enters the public domain and is free for all to use without authorization [31]. This issue, however, can be modeled by a distinction between private and public data (or protected and non-protected data). Second, to achieve its constitutional goals, copyright law excludes certain subject matter from legal protection as they are considered as the “raw material” needed for cultural expression by other creators. According to the US Supreme Court, “originality” is “[t]he sine qua non of copyright.” [Feist Publ’ns, Inc. v. Rural Tel. Serv. Co., 499 US 340, 345 (1991).] Accordingly, only the original elements within copyrighted works are legally protected by copyright law. Unoriginal elements (e.g., ideas, facts) are never protected. Privacy, by contrast, seeks to protect content and not merely an original expression, which, in turn, can be misaligned with the fundamental purpose of the law. This point cannot be overestimated. Copyright law does not only allows subsequent authors to draw upon the unoriginal, and thus unprotected, elements of copyrighted works (unlike in privacy), it encourages subsequent authors to do so (Jessica D. Litman, The Public Domain, 39 EMORY L.J. 965, 975 (1990) Niva Elkin-Koren, Copyright in The Digital Ecosystem: A User Rights Approach, in COPYRIGHT LAW IN AN AGE OF LIMITATIONS AND EXCEPTIONS 132 (Ruth Okediji ed., 2017)). Because copyright protection only applies to some elements within copyrighted works (i.e, expression) while deliberately excluding others (i.e., ideas) courts need to delineate the scope of legal protection when deciding copyright disputes. As a result, the scope of copyright protection varies not only among different works but also among different elements within a single work (SAS Institute Inc. v. World Programming Ltd., 64 F. Supp. 3d 755, 762 (E.D.N.C. 2014)).  
Third, in a stark distinction from privacy, copyright law also encourages the use of the original (and thus protected) elements of copyrighted works in certain circumstances. These include de minimis quotations, transformative uses serving different purposes compared to the purpose of the original work (such as parodies), and many other types of “fair uses” such as learning and research [33]. The fair use doctrine serves as a check on copyright, ensuring it does not stifle the creativity copyright law seeks to foster. Fair use is also considered one of the safety valves that allow copyright protection to coexist with freedom of expression [32]. 
For all these reasons, privacy notations are both over-inclusive and under-inclusive from a copyright perspective. They are over-inclusive because they withhold much more from subsequent authors than copyright law necessitates, consequently undermining the objectives of copyright law. At the same time, by focusing on content rather than original expression, privacy notations are also under-inclusive because they allow (in some cases) unlawful access to original copyrighted expression. This could happen, for example, if Alice’s model did not access input content B, but did access input content C that incorporated original expression deriving (lawfully or not) from input content B. 
In this work, we discuss the challenges involved in providing a rigorous definition that captures the concept of copyright. We begin by formally comparing various proposed interpretations of copyright, particularly focusing on  differential privacy and NAF), and examine their close connection to algorithmic stability. Subsequently, we argue that any approach adhering to this line of reasoning encounters significant obstacles in accurately modeling copyright as defined within the legal framework. In more detail, we identify several major gaps between algorithmic stability strategies and copyright doctrine and demonstrate why applying these strategies overlook certain crucial aspects of copyright law, which are designed to maintain its delicate balance. 
Based on this analysis, we argue that if algorithmic stability techniques are adopted as a standard for copyright infringement, they may undermine copyright law's constitutional mandate and intended goals. We propose future research to focus on limiting algorithmic stability strategies to expressive “elements” rather than content and suggest using such strategies to inform copyright originality rather than for assessing infringement. 



\subsection{Related Work}

A growing number of researchers in recent years have explored how to address legal problems by applying theories and methods of computer science. This literature seeks to narrow the gap between the vague and abstract concepts used by law and use mathematical models to offer more rigor, coherent, and scalable definitions of issues such as privacy [19] or fairness and discrimination [21, 27]. In the context of generative models, Carlini et al. [17] and Haim et al. [25] explore whether generative diffusion models memorize protected works that appeared in the models’ training set. Such memorization may, in some cases, be indicative of copyright infringement. However, as discussed, memorizing an input content does not necessarily equate with copyright infringement. For this reason, a more nuanced and accurate analysis calls for developing measurable metrics for copyright law’s key limiting concepts (i.e., original, idea/expression, fair use). We discuss this option in Section 4. 
There is also active and thought-provoking discussion on how ML technologies are reshaping our understanding of copyright law. For example, Asay [14] explores the question of whether AI system outputs should even be subject to copyright protection. These policy questions exceed the scope of this paper. The works of Grimmelmann [24] and Lemley and Casey [30] reflects on copyright law’s requirement of human authorship and fair use for the purpose of machine learning. Our focus, though, is on the legitimacy of using AI for generating synthetic content. Most relevant to our project are the works of Bousquet et al. [15] and Vyas et al. [38], both rely on privacy/privacy-like notions to inform copyright infringement analysis. 
Alternative approaches were considered by Scheffler et al. [36] and by Franceschelli and Musolesi [23]. Scheffler et al. [36] proposed a framework to test substantial similarity in copyright infringement analysis by comparing Kolmogorov-Levin complexity with and without access to the original copyright work.  However, to properly apply a substantial similarity test, one  must first distinguish between protected (original) expression and unprotected (unoriginal) ideas. We argue that this is a crucial and overlooked challenge. Another approach by Franceschelli and Musolesi [23] suggests using generative learning techniques to assess creativity. Such approaches my prove valuable as we suggest in Section 4, but only if they are designed to align with copyright principles.  
Lastly, Henderson et al. [26] develop strategies for generative models to ensure they satisfy the same fair use standard as in human discretion. The application of this solution may not be possible, however, in cases where little to no open-source or fair-use data is readily available.




\section{Algorithmic stability as a surrogate for copyright}
In this section, we focus on introducing and discussing two notions of algorithmic stability: near-access freeness (NAF) and differential privacy (DP); these two notions were  explicitly investigated in the realm of training methods aimed at safeguarding copyrighted data.
Both NAF and DP adhere to a shared form of stability: they ensure that the resulting model, denoted as q, satisfies a safety condition with respect to each copyrighted data instance, denoted as c. This safety condition guarantees the existence of a “safe model,” denoted by qc, which does not infringe the copyright of data c, and importantly, q exhibits sufficient similarity to qc. Consequently, both NAF and DP guarantee that p itself does not violate the copyright of the respective data instance c.
Formally, we consider a standard setup of an unknown distribution D and a generative algorithm A. The algorithm A gets as an input a training set of i.i.d samples S = {z1,...,zm} ∈ Zm ∼ Dm, and outputs a model pAS = A(S), which is a distribution supported on Z. For simplicity, we will assume here that Z is a discrete finite set, but of arbitrary size. Vyas et al. [38] consider a more general variant in which the output posterior is dependent on a “prompt” x, and A outputs a mapping p(AS)(·|x) that may be regarded as a mapping from prompts to posteriors. For our purposes, there is no loss in generality in assuming that p is “promptless”, and our results easily extend to the promptful case by thinking of each prompt as inducing a different algorithm when we hard-code the prompt into the algorithm.


\paragraph{Differential Privacy} %A well-studied notion of stability in this context is that of differential privacy \cite{dwork2018privacy}. 

$A$ is said to be $(\alpha,\beta)$-differentially private \cite{dwork2006calibrating} if for every pair of input datasets $S,S'$ 
that differ on a single datapoint, we have that for every event $E$:
\begin{equation}\label{eq:privacy} 
\P(A(S) \in E) \le e^{\alpha} \P(A(S')\in E) + \beta \text{ and } \P(A(S') \in E) \le e^{\alpha} \P(A(S)\in E) + \beta
\end{equation}
The concept of privacy, viewed as a measure of copyright, can be explained as follows: Let’s consider an event, denoted as E, which indicates that the generative model produced by A violates the copyright of a protected content item c. The underlying assumption (which is criticized below) is that if the model has not been trained on c, the occurrence of event E is highly improbable. Thus, we can compare the likelihood of the event E when c is present in the sample S with the likelihood of E when c is not included in a neighboring sample S′ (which is otherwise identical to S). If A satisfies the condition stated in equation Eq. (1), then the likelihood of event E remains extremely low, even if c happened to be present once in its training set.


% The interpretation of privacy as a copyright measure can be thought of as follows: consider an event $E$ which represents that the generative model $p$ that $A$ outputs violates the copyright of some protected content $z$. The underlying assumption here is that if $p$ has not been trained on $z$ then the event $E$ is highly unlikely. In turn, we compare the likelihood of the event $E$ when $z$ is \emph{in} the sample $S$ to that of a neighboring sample $S'$ that does not include $z$ (but otherwise is identical to $S$). Then, if $A$ satisfies \cref{eq:privacy} then the likelihood of $E$ remains very low, even if $z$ did appear once in its training set.


\paragraph{Near Access  Freeness} . There are several shortcomings of the notion of differential privacy that have been identified. Some of these are reiterated in Section 3. Vyas et al. [38] proposed the notion of Near-Access Freeness (NAF) that relaxes differential privacy in several aspects. Formally, NAF (or more accurately, NAF w.r.t safe function safe and ∆max is defined as follows: First, we assume a mapping safe that assigns to each protected content c a model qc, which is considered safe in the sense that it does not breach the copyright of c. The function safe, for example, can assign c to a model that was trained on a sample that does not contain c. Several safe functions have been suggested in [38].
A model p is considered α-NAF if the following inequality holds simultaneously for every protected content c and every z:

\begin{equation}\label{eq:naf}
p (z) \le e^{\alpha} q_{c}(z).
\end{equation}

The intuition behind NAF is very similar to the one behind DP; however, there are key differences that can, in principle, help it circumvent the stringency of DP.

\begin{enumerate}
    \item1.	The first difference between NAF and DP is that the NAF framework allows more flexibility by picking the ’safe’ function. Whereas DP is restricted to a safe model corresponding to training the learning algorithm on a neighboring sample excluding the content c.
    % Our focus here will be on \emph{sharded safety} that divides the sample into two subsamples and assigns to each content $z$ a safe model which was trained on the subsample that does not contain $z$.
    \item A second difference is the fact that NAF is one-sided (see Eq. (2)), in contrast with DP, which is symmetric (see Eq. (1)). Note that one-sidedness is indeed more aligned with the requirement of copyright, which is non-symmetric.
    \item3.	NAF makes the distinction between content-safety and model-safety [38]. In more detail, the NAF notion requires that the output model is stable. This contrasts with privacy, which requires stability of the posterior distribution over the output models. In this sense, the notion of NAF is more akin to prediction differential privacy [19] than to differential privacy.
    \item Finally, NAF poses constraints on the model outputted by the learning algorithm (each constraint corresponds to a prespecified safe model). This contrasts with privacy, which does not restrict the output model but requires stability of the posterior distributions over output models. This distinction may seem minor, but it can lead to peculiarities. For example, an algorithm that is entirely oblivious to its training set and always outputs original content can still violate the requirements of NAF. To see this, imagine that our learning rule outputs a model q that always generates the same content z, which is entirely original and not similar to any protected content c. However, depending on the safe models qc it can be the case that the model q is not similar to any of them.
    
    %In fact, it can do so even if it outputs completely original content. 
    %and outputs a completely original content, may still be deemed not NAF.
\end{enumerate}


The above differences potentially allow NAF to circumvent some of the hurdles for using DP as a notion for copyright. For example, the one-sidedness seems sufficient for copyright and may allow models to be discarded via DP. Also, the distinction between model-safety and content-safety can, for example, enable models that completely memorize the training set as long as the content they output does not provide proof for such memorization. Next, the fact that NAF is defined by a set of constraints and not a property of the learning algorithm allows one to treat breaches of Eq. (2) as soft “flagging” and not necessarily as hard constraints. This advantage is further discussed in Section 4. Finally, perhaps most distinguishable, is the possibility of using general safety functions that can capture copyright breaches more flexibly. We next discuss the implications of these refinements. We begin with the question of model safety vs. content safety in NAF and DP.

\paragraph{Model safety vs. Content safety}
safety Our first result is a parallel to Theorem 3.1 in [38] in the context of DP stability. Theorem 3.1 in [38] shows how to efficiently transform a given learning rule A to a learning rule B, which is NAF-stable, provided that A tends to output similar generative models when given inputs that are identically distributed. We state and prove a similar result by replacing NAF stability with DP stability.
Recall that the total variation distance between any two distributions is defined as:



% Our first result shows that analogously to NAF one can relax the notion of DP and require only content safety and achieve similar guarantees. \cref{thm:main_up} shows that when an algorithm has non-trivial TV stability then its output content can be privatized. This can be seen as an analogue to Theorem 3.1 in \cite{barak} which proved a parallel result for NAF. We point out, that similar to the guarantee in NAF, we do not publish a private model that is close in total variation to the original model. Instead we provide a private estimate of a model that is close in total variation to the original mode. By sampling from this model, we obtain a single content that is sampled from a distribution that is close to the original model as in NAF.

Recall that the total variation distance between any two distributions is defined as:
$ \|q_1-q_2\| = \frac{1}{2}\sum |q_1(x)-q_2(x)|= \sup_{E} \left(q_1(E)-q_2(E)\right),$
\begin{proposition}\label{thm:main_up}
    Let $A$ be an algorithm mapping samples $S$ to models $q^A_S$ such that
    \[ \E_{S_1,S_2}\left[\| q^A_{S_1}- q^A_{S_2}\|\right] \le \alpha,\]
    where $S_1,S_2\sim D^m$ are two independent samples.
    Then, there exist an $(\epsilon,\delta)$ DP algorithm $B$ that receives a sample $S_B\sim D^{m_{priv}}$ such that if $m_{priv} = \tilde O\left(\frac{m}{\eta\epsilon}\log 1/\delta\right)$  and $S_A\sim D^m$ then:
    \[  \E_{S_A,S_B}\left[\|\E[q^B_{S_B}]- q^A_{S_A}\|\right] \le \frac{2\alpha}{1+\alpha}+O(\eta).\]
    Where the expectation within, is taken over the randomness of $B$.
\end{proposition}
The premise in the above theorem is identical to that in Theorem 3.1 in~\cite{barak} and captures the property that $A$ provides similar outputs on identically distributed inputs. The obtained algorithm $B$ is DP-stable and at the same time it has a similar functionality like $A$ in sense that its output model $q^B$ generates content $z$ which in expectation is distributed like contents generated by $q^A$.

\paragraph{Safety functions}
We now turn to a discussion on the potential behind using different safety functions. The crucial point (which we discuss in great detail in Section 3 below) is that a satisfactory “copyright definition” must allow algorithms to be highly influenced, even by their input content, which is protected. This starkly contrasts algorithmic stability: it is easy to see that DP does not allow such influence. Indeed, the philosophy behind privacy is that a model is “safe” if it does not observe the private example (and in particular, is not influenced by it).
This raises the question of whether the greater flexibility of the NAF model can provide better-aligned notions of safety. In fact, if it is allowed to be influenced by protected data, one might even want to consider safe models that have intentionally observed a certain content and derived out of it the derivatives that are not protected.
The following result, though, shows that there is a no free lunch phenomenon. For every protected content c, we can either only consider safe models that observed c and are influenced by it or only safe models that never observed it and were not affected by it. In other words, if a protected content c influenced its safe model qc, then it must influence all safe models qc′ for all protected contents c′. We further elaborate on the implication of this result in Section 4.
Below, q1 and q2 should be thought of as safe models, and p as the model outputted by the NAF learning algorithm. (So, in particular, p should satisfy Eq. (2) w.r.t q1 and q2.) This result complements Theorem 3.1 in [38], which shows that NAF can be satisfied in the sharded-safety setting when the two safe models are close in total-variation
\begin{proposition}\label{thm:main_low}
Let $q_1$ and $q_2$ be two distributions such that
$ \|q_1-q_2\|\ge \alpha,$
then for any distribution $p$ we have that for some $z$:
\[ p(z) \ge \frac{1}{2(1-\alpha)} \min\{q_{1}(z),q_{2}(z)\},\]
\end{proposition}


% Notice, that the result does not assume anything about $p$, nor on the definition of $\safe$. 
% Thus, we are faced with two alternatives. Either for each protected content $c$ we hold a safe model $q_{c}$ that allows influences of $c$ on the output content of the types considered in \cref{sec:law}, or we hold a safe model that did not observed $c$. However, both cannot be considered safe. The implications of this are further discussed in \cref{sec:discussion} after we address the gap between algorithmic stability and copyright.


%\cref{thm:main_low,thm:main_up} state, respectfully, that for ``NAFification", a necessary condition is non-trivial TV-stability, and TV-stability allows also privatization. In other words, any model that is NAF is similar, in terms of their output content, to a model that is private.
%As discussed, the reverse is not true. For example an algorithm that is oblivious to the sample is private by definition. Whether it is NAF or not depends on the safety function.

 %Our formal result shows that any NAF model is close to a private model. The closeness scales with the stability of the algorithm $A$ which may be non trivial but far from $1$. In both NAF and \cref{thm:main_up} the TV stability, though, controls the degradation, i.e. how close the new model is to the original (potentially copyright infringing) model which is regarded as the utility of the algorithm. 
 %\textcolor{red}{I don't quite understand this paragraph}


\ignore{
\paragraph{Model safety vs.\ content safety} 
    As discussed a NAF algorithm outputs a content $z$ from a model $p$ that is ``safe". DP is a property of the output posterior $p$. In other words, $p$ may be NAF even though $p$ itself (and not a single content drawn from $p$) reveals the input content. \cref{thm:main_up}, though, shows that any NAF model is close to a model that in itself does not reveal the input content. As such, this relaxation does not necessarily allow a better aligned notion of copyright.
    
    We can also interpret the DP algorithm $B$ as sampling $z$ from $\E[q^B_S]$. Under this interpretation we obtain a DP guarantee for the output content $z$ analogously to NAF. However, the result we obtain is stronger, in the sense that it allows one to output the whole model $q_S^B$.}
\ignore{   
\paragraph{Alternative NAFs:} As discussed, we focused here on NAF with respect to sharded safety and $\Delta_{max}$. Alternative notions allow weaker metrics to measure degradation (such as the KL divergence) and alternative notions of safety. With $KL$ divergence one can obtain NAF algorithms whose parameter scale with the \emph{Hellinger squared distance}, $H(p,q_S)$,  instead of total variation. However, given the well known relation:
$ H^2 (p,q)\le \|p-q\| \le \sqrt{2}H(p,q),$
qualitatively, we can obtain analogous results. Another interesting notion is that NAF with respect to leave-one-out safeness, which is distinct from cDP in its one-sidedness. It is interesting whether this one-sideneness indeed opens up the possibility to alternative metrics for copyright.
\paragraph{Statistical/algorithmic separation} It is important to note that we did not focus here on the statistical or algorithmic implications of the use of NAF. It is an important, an interesting question, whether NAF allows more scalable techniques to obtain safe models. Our focus here is to study what is regarded as ``safe" in the NAF sense vs. the DP sense. 
}
\section{The gap between algorithmic stability and copyright}\label{sec:law}
So far, we provided a technical comparison between existing notions in the CS literature aimed towards provable copyright protection. While the technical notion of privacy may seem closely related, as observed through NAF, there are differences, and there is room for more refined definitions that may capture essential differences. While algorithmic stability approaches hold promise in helping courts assess copyright infringement cases (an issue we further discuss in Section 4), as we discuss below, such methods cannot serve as a definitive test for copyright infringement. To see why, we next discuss the issue of copyright through the lens of the law. From a legal perspective, formal algorithmic stability approaches are both over and under-exhaustive. Consequently, we will categorize this section based on these challenges.

%


\subsection{Over-inclusiveness }
Here, we focus on a concern that algorithmic stability approaches may filter out lawful output content that does not infringe copyright in the input content. Because non-infringing output content is lawful, employing algorithmic stability approaches as filters to generative models may needlessly limit their production capabilities and, thereby, undermine the goals of copyright law.
Copyright law intends to foster the creation of original works by securing incentives for authors while ensuring the freedom of current and future authors to use and build upon existing works. The law derives from the US Constitutional authority: “To promote the Progress of Science and useful Arts, by securing for limited Times to Authors and Inventors the exclusive Right to their respective Writings and Discoveries.” [5]
However, the goal of promoting progress is inconsistent with unlimited rights to control copyrighted materials. For this reason, copyright law sets fundamental limits on the rights it grants to authors. Promoting progress is incompatible with absolute rights to control copyrighted materials because creators and creative processes are situated in a cultural and cumulative context. The creative process often involves an ongoing interaction with multiple stakeholders rather than authorship in silos. Creating new works involves human capital enhanced by learning and research, engagement with pre-existing materials, and a shared cultural language. Consequently, using copyrighted materials is an essential input in any creative process. Such a process often involves learning from pre-existing materials, applying existing styles, and referencing shared symbols and common works to generate new interpretations and fresh meanings [18, 22].
For this reason, unlike the mandate of the algorithmic stability approaches, copyright law does not require that output content will not draw at all on input content to be lawful and non-infringing. On the contrary, there are many cases where copyright law explicitly allows output content to draw heavily on the input content without raising infringement concerns. In such cases, allowing input content to impact output content is not only something copyright law permits, it is something copyright law encourages. Doing so, as Jessica Litman put it: “is not parasitism; it is the essence of authorship.” [31]
Copyright law allows an output content to substantially draw on input content in three main cases. We list and then explore these categories:

(1) When the input content is in the public domain, (2) When the input content is copyrighted but incorporates aspects that are excluded from copyright protection, and (3) When the use of the protected aspects of the input content are lawful.



\paragraph{When an input content is in the public domain}
Input content may be unprotected because its copyright term has lapsed. Copyrights are limited in duration (though relatively long duration, which in most countries will last the life of the author plus seventy years). Once the copyright term expires, input content enters the public domain and can freely be used and impact output content without risking copyright infringement [31]. Public domain materials may also contain anything that is not copyrightable at all, such as natural resources. For instance, if two photographers are taking a picture of the same person, some similarity between the pictures might be due to how this person looks, which is in the public domain. Other elements, such as an original composition or the choices made regarding lighting conditions and the exposure settings used in capturing the photograph, may be considered copyrighted expression. If the generative model only uses the former in the output content, it may not constitute an infringement.


\paragraph{When an input content incorporates unprotected aspects}
. Input contents with a valid copyright term, enjoy “full” legal protection, but it too is limited in scope. As provided by the copyright statute, “[i]n no case does copyright protection for an original work of authorship extend to any idea, procedure, process, system, method of operation, concept, principle, or discovery, regardless of the form in which it is described, explained, illustrated, or embodied in such work.” [1] According to this principle, an output content may substantially draw on an input content without infringing the latter’s copyrights, for as long as such taking is limited to the input’s content unprotected elements.



\begin{itemize}
    \item \textbf{Procedures, processes, systems and methods of operation}
Copyright protection does not extend to “useful” or “functional” aspects of copyrighted works, such as procedures, systems, and methods of operation. These aspects of input content are freely accessible for output content to draw upon. For example, in the seminal case of Baker vs. Selden, the Supreme Court allowed Baker to create a book covering an improved book-keeping system while drawing heavily on the charts, examples, and descriptions used in Selden’s book without infringing Selden’s copyright [3]. As the court explained, the aspects that Baker took from Selden’s work are functional methods of operations and, as such, are not within the domain of copyright law. Similarly, in Lotus v. Borland, the United States Court of Appeals for the First Circuit allowed Borland to copy Lotus’s menu command hierarchy for its spreadsheet program, Lotus 1-2-3. The court ruled that the Lotus menu command hierarchy was not copyrightable because they form methods of operation [8]. Consequently, if generative models simply extract procedures, processes, systems and methods from the training set, they will not infringe copyright.

    \item \textbf{Ideas}
    
    Copyright protection is limited to concrete “expressions” and does not cover abstract “ideas.” Thus, in Nicholas v. Universal, the United States Court of Appeals for the Second Circuit allowed Universal to incorporate many aspects of Anne Nichols’ play Abie’s Irish Rose in their film The Cohens and Kellys [11]. The court explained that the narratives and characters that Universal used (“a quarrel between a Jewish and an Irish father, the marriage of their children, the birth of grandchildren and a reconciliation”) were “too generalized an abstraction from what she wrote. . . [and, as such]. . . only a part of her [unprotected] ‘ideas.’” [11] When a generative model extracts ideas from copyrighted materials rather than replicating expressive content from their training data, it does not trigger copyright infringement.

    \item \textbf{Facts}
 Copyright protection also does not extend to facts. For example, in Nash v. CBS, the court ruled that CBS could draw heavily from Jay Robert Nash’s books without infringing his copyright [10]. As the court explained, the hypotheses that Nash rose speculating the capture of the gangster John Dillinger and the evidence he gathered (such as the physical differences between Dillinger and the corpse, the planted fingerprints, and photographs of Dillinger and other gangsters in the 1930s) were all unprotected facts that Nash could not legally appropriate. Consequently, generative models which memorize facts do not infringe copyright law.
\end{itemize}

\paragraph{When the use of the protected aspects of the input content was lawful}
Even when the protected elements of an input content (“expressions” rather than the “ideas”) are impacting an output content, such impact may be legally permissible. There are two main categories of lawful uses: de minimis copying and fair use.


\begin{itemize}
    \item \textbf{De minimis copying} 
  Copyright law allows de minimis copying of protected expression, namely the coping of an insignificant amount that has no substantial impact on the rights of the copyright owner or their economic value. Similarly, “[w]ords and short phrases, such as names, titles, and slogans, are uncopyrightable.”[37]. However, de minimis copying of protected expression may be unlawful if it captures the heart of the work [4]. For example, phrases like “ET Phone Home.” [12]
    \item \textbf{Fair Use}
   Use Copyright law also allows copying protected expression if it qualifies as fair use. The US fair use doctrine, as codified in § 107 of the US Copyright Act of 1976, is yet another legal standard to carve out an exception for an otherwise infringing use after weighing a set of four statutory factors. The four statutory factors are (1) the purpose and character of the use, including whether such use is commercial or is for nonprofit educational purposes; (2) the nature of the copyrighted work; (3) the amount and substantiality of the portion used in relation to the copyrighted work as a whole; and (4) the effect of the use upon the potential market for or value of the copyrighted work [1].

\end{itemize}
Notably, the fair use claimant does not need to satisfy each factor for the use to qualify as fair use [7]. Nor are the four factors meant to set out some mathematical equation whereby, if at least three factors favor or disfavor fair use, that determines the result [33]. Rather, the factors serve as guidelines for holistic, case-by-case decisions. In that vein, in its preamble paragraph, § 107 lists several examples of the types of uses that can qualify as fair use. The examples, which include “criticism, comment, news reporting, teaching (including multiple copies for classroom use), scholarship, [and] research,”[1] are often thought to be favored uses for qualifying for fair use. Importantly, however, the list of favored uses is not dispositive. Rather, fair use’s open-ended framework imposes no limits on the types of uses that courts may found “fair” [7].
When the factors strongly favor a finding of fair use, even output contents that are heavily impacted by copyrighted input contents may be excused from copyright infringement. For example, in Campbell v. Acuff-Rose, although the rap music group 2 Live Crew copied significant portions of lyrics and sound from Roy Orbison’s familiar rock ballad “Oh, Pretty Woman” [7], the Supreme Court denied liability. The court reasoned that 2 Live Crew’s derivative work was considered a “parody” of Orbison’s original work and, therefore, constituted fair use. Similarly, in The Authors Guild v. Google, the court defended Google’s mass digitization of millions of copyrighted books to create a searchable online database as fair use because it considered Google’s venture socially desirable [2]. As explained by Sag [34], copying expressive works for non-expressive purposes should not be counted as a copyright infringement and be likely to be considered fair use.

 
\subsection{Overly Exclusiveness}
Algorithmic stability approaches are under-exhaustive because they might fail to filter out unlawful output content that infringes copyright in the input content. As explained, algorithmic stability approaches find infringement only when the output content heavily draws on input content. The law of copyright infringement, however, is not so narrow. Copyright law only requires that the output content heavily draw on the protected expression originating from an input content to find infringement. Such expression need not necessarily come from the input content itself; it may come from various other sources, including copies, derivatives, or snippets of the original content.
To illustrate this point, consider the fact pattern in the pending Supreme Court case Warhol vs. Goldsmith [6]. In that case, the portrait photographer Lynn Goldsmith accused Andy Warhol of infringing copyrights in a photograph she took of the American singer Prince. Goldsmith consented to Warhol to use her photograph as an “artistic reference” for creating one derivative illustration.  Still, she did not approve nor imagine that Warhol had made 16 different derivative images from the original photograph. Warhol’s collection of Prince portraits, also known as the Prince series, is depicted in Fig. 1, right side.
For our purposes, assume the Prince Series’ portraits served as input for a generative machine. Suppose the machine’s output content draws heavily on Goldsmith’s protected expression that is baked into the Prince Series’ portraits. In that case, the output content may infringe Goldsmith’s copyright in the original photograph (Fig. 1, left side), even if the machine did not have access to Goldsmith’s original photograph. This risk will not be eliminated even if the Supreme Court decides that the Prince Series’ portraits themselves are non-infringing as they constitute fair use.
Simply put, copying from a derivative work—whether authorized by the copyright owner or not— may infringe copyright in the original work on which the derivative work is based. This situation is prevalent in copyright practice, especially in music.
In modern music copyright cases, plaintiffs usually show access to the original copyrighted work (musical composition) by showing access to a derivative work of that original work (sound recording). Plaintiffs are not required to demonstrate that the defendants also had access to the original sheet music nor that they could actually read musical notes.
Lastly, output content can also infringe copyright in input content by accessing parts or snippets of the input content even without accessing the input content in its entirety. This concern was raised in The Authors Guild v. Google, a case dealing with the legality of the Google Book Search Li-
	Figure 1	brary Partner project [2]. As part of this project,
Google scanned and entered many copyrighted books
into their searchable database but only provided “snippet views” of the scanned pages in search results to their users. The plaintiff in the case argued that Google facilitated copyright infringement by allowing users to aggregate different snippets and reconstruct infringing copies of their original works. The court ended up dismissing this claim, but only because Google took affirmative steps to prevent such reconstruction by limiting the number of available snippets and by blacklisting certain pages.
To sum up, there are numerous instances where copyright law permits (even encourages) an output content to draw upon an input content. The more substantial the unprotected aspects of input content, and the more likely it is that using the input content’s protectable aspects is considered lawful, the more expansively can the output content draw on the input content without fearing copyright liability. At the same time, there are cases where copyright law outlaws an output even if it did not draw upon an input content, provided that it did draw on protected expression that originated from that content. The more original the input content, and the more copies, derivatives, or snippets of that original content exist in the model datasets, the more likely the output content is to infringe copyrights in that input content. Therefore, any strategy for detecting or mitigating copyright infringement must account for these crucial copyright distinctions.   




\section{Discussion}\label{sec:discussion}
Algorithmic stability approaches establishing proof of copyright infringement are both too strict or too lenient from a legal perspective. Due to this misfit, applying algorithmic stability approaches as filters for generative models will likely distort the delicate balance that copyright law aims to achieve between economic incentives and access to creative works.
		Stability is not safe. It is crucial to understand the limitations of algorithmic stability approaches. The NAF framework, which allows a rich class of safety functions, has the potential to circumvent some of the challenges presented. Nevertheless, this framework still fails to adhere to copyright principles. To utilize the NAF framework, the first fundamental question one needs to address, is

Given a protected content c, how should we choose the safe model safe(c)?
It seems natural to include models not heavily influenced by c since otherwise, this might allow copyright breaching. However, such a choice of safe(c) leads to the same limitations encountered by the DP setting. It is true that some aspects, such as content safety vs. model safety, can be better aligned through the definition of NAF but also, as Proposition 1 shows, through variants of DP. Overall, there is room, then, to further investigate the different possible models for copyright, within such an approach, but we should take into account the limitations presented in Section 3.
Perhaps a more exciting application of NAF, then, is to consider notions of safety that allow some influence by c. For example, to enable generating parodies, fair use, de minimis copying, etc. We  then consider safety functions that now have access to c and exploit this access to validate that only permissible influence happens. Here, we face a different challenge. Suppose that qc is such a safe model for content c. Suppose, also, that qc′ is another safe model for content c′. If qc′ and qc are far away, then Proposition 1 shows that there is no hope to output a NAF model. But even if qc and qc′ are not far away, but suppose that qc′ ignores content c, then for any content z that is influenced by c, we may assume that:
qc(z) ≫ qc′(z).
But, if p is a NAF model, we must also have due to Eq. (2) with respect to c′ and z:
qc(z) ≫ p(z).
In other words, the NAF model censors permissible content z even though it is safe. This happens because z is an improbable event in model qc′. Not because z breaches the copyright of c′ but because it is influenced by c, and content that is influenced by c is discarded by safe models that had no access to c.
It follows, then, that all safe models must treat protected content in a similar manner, and qc′ must also be influenced by c if we expect the NAF model to make any use of it. Hence, it is unclear if a more refined notion of safe may help circumvent the hurdles of the privacy approach. This suggests, though, to perhaps consider a relaxed variant of NAF in which content is discarded by a safe model only when certain links between the protected content and the generated content are established.
It seems that an algorithmic approach that assists jurists in understanding such links between existing works of authorship, studying their hidden interconnection, and quantifying their originality can hold great promise. In other words, rather than constructing binary legal rules (e.g., aiming to devise a definitive test for copyright infringement), algorithmic stability approaches could facilitate new quantifiable methods for applying legal standards, such as measuring originality [Uri Y. Hacohen & Niva Elkin-Koren, Copyright Regenerated: Harnessing GenAI to Measure Originality and Copyright Scope, 37(2) Harv. J. of L& Tech. (2024)]. From this perspective, originality is evaluated by the semantic distance between the elements of a measured expressive work and similar elements found in the corpus of the training content. . The more salient the expressive elements within the larger corpus of pre-existing content, the less likely these elements are to be considered original by copyright law, and the more likely copyright law is to legitimize drawing upon them by the output content.
Research in this area is still in its infancy but holds grand promise for the copyright system [W. Shi, A. Cui, E. Li, R. Jia, and Z. Yu. Selective differential privacy for language modeling. In Conference of the North American Chapter of the Association for Computational Linguistics: Human Language Technologies, 2022.; Valentin Hartmann, Anshuman Suri, Vincent Bindschaedler, David Evans, Shruti Tople, & Robert West, SoK: Memorization in General-Purpose Large Language Models,(….)]. Algorithmic approaches that focus on the element level rather than the content level, and are applied not as binary tests for apprising infringement but as tools for measuring copyright originality may greatly empower the legal profession. As the extensive  body of legal scholarship has long acknowledged, the originality standard in copyright law, along with many of its related doctrines for delineating scope (such as the “idea-expression dichotomy”), is inherently vague and uncertain[Jessica D. Litman, The Public Domain, 39 EMORY L. J. 965, 975 (1990); Mark A. Lemley, Our Bizarre System for Proving Copyright Infringement, 57 J. Copyright Soc’y 719, 748 (2010); Richard H. Jones, The Myth of the Idea/Expression Dichotomy in Copyright Law, 10 PACE L. REV. 551, 553 (1990)]. Such vagueness leads to inconsistent judicial precedent, deters permissible uses of copyrighted material, and undermines the goals of copyright law. [James Gibson, Risk Aversion and Rights Accretion in Intellectual Property Law, 116 Yale L. J. 882, 884 (2007); Neil W. Netanel, Introduction, Copyright’s Paradox 54-80 (2008) 7 (UCLA School of Law, Research Paper No. 08-06, 2008); Jessica D. Litman, Billowing White Goo, 31 COLUM. J. L. & ARTS 587, 587 (2008); Pamela Samuelson, The Copyright Grab, WIRED (Jan. 1, 1996) https://www.wired.com/1996/01/whitepaper/; SIVA VAIDHYANATHAN, COPYRIGHTS AND COPYWRONGS: THE RISE OF INTELLECTUAL PROPERTY (2003)].



 
